SA4U: Practical Static Analysis for Unit Type Error Detection

Unit type errors, where values with physical unit types (e.g., meters, hours) are used incorrectly in a computation, are common in today's unmanned aerial system (UAS) firmware. Recent studies show that unit type errors represent over 10% of bugs in UAS firmware. Moreover, the consequences of unit type errors are severe. Over 30% of unit type errors cause UAS crashes. This paper proposes SA4U: a practical system for detecting unit type errors in real-world UAS firmware. SA4U requires no modifications to firmware or developer annotations. It deduces the unit types of program variables by analyzing simulation traces and protocol definitions. SA4U uses the deduced unit types to identify when unit type errors occur. SA4U is effective: it identified 14 previously undetected bugs in two popular open-source firmware (ArduPilot & PX4.)

==> ii_nutshell_copy.tex <==
\section{SA4U in a Nutshell}
\begin{figure}
    \centering
    \includegraphics{figures/overview.pdf}
    \caption{SA4U's workflow. The boxes show each stage of SA4U's execution. Components shown in gray are not part of SA4U. Icons show the inputs and outputs of each stage.}
    \label{fig:SA4U_Overview}
\end{figure}

In this section, we motivate the issue of unit type errors and show the operation of SA4U with a real-world example.

\subsection{Challenges}
SA4U aims to identify unit type errors without any annotation burden. While it is possible to use type inference to learn the types of program variables, inference is only possible if \emph{some} variables have types that are known to begin with. SA4U addresses this challenge in two ways. First, SA4U uses existing protocol definition files that describe the messages sent between the pilot's control computer and the UAS. Second, SA4U mines the history of values written to program variables to deduce the variable's type.

Both type sources introduce new challenges. Protocol definition files contain messages with fields whose type depends on the value of another field. To date, no analysis tool handles this case. Second, UAS firmware is sensitive to timing perturbations. The mechanism SA4U uses to obtain the history of variable writes must be careful to avoid changing the behavior of the firmware. 

\subsection{Motivating Example}
% Figure \ref{fig:Instrumented_Source_Code} shows a simplified version of ArduPilot's message handler for external vision speed estimates. The message handler in \code{on\_vsn\_spd\_est} invokes the \code{correct\_time} method to account for transport delay of the message. Part of the logic of \code{correct\_time} is shown in Figure \ref{fig:Instrumented_Source_Code}. The expected remote time is computed on line 14. Then, the difference between the expected remote time and received remote time is computed on line 16. The bug here is simple: the message handled by the logic in Figure \ref{fig:Instrumented_Source_Code} can have a \code{usec} member formatted in either UNIX time (i.e. the number of seconds since January 1, 1970) or time since the UAS booted, but the handler fails to distinguish between the two timestamp formats. The remote computer is at liberty to supply values in \emph{any} timestamp format. But switching timestamp formats causes a nonsensical computation on line 16.

Figure \ref{fig:Instrumented_Source_Code} shows a simplified version of ArduPilot's message handler for obstacle distances. A separate system onboard the UAS detects obstacles and communicate their distances to the main flight controller with this message. Execution of the message handler starts on line \ref{fig:Instrumented_Source_Code:1}. The handler performs some processing of the message and then invokes the \lstinline{set_obstacle_boundary} function on line \ref{fig:Instrumented_Source_Code:2} with the message's \lstinline{angle} and \lstinline{distance} fields. The body of \lstinline{set_obstacle_boundary} assigns these fields to the \lstinline{_angle} and \lstinline{_distance} fields on lines \ref{fig:Instrumented_Source_Code:angle_assgn} and \ref{fig:Instrumented_Source_Code:dist_assgn}. This is a bug, since the program variable \lstinline{_angle} is measured in the vehicle's reference frame. Meanwhile, \lstinline{msg}'s members could be relative to \emph{any} reference frame. After consulting with ArduPilot's developers, we created the patch shown on line \ref{fig:Instrumented_Source_Code:patch}. ArduPilot does not mean to support coordinate systems other than the vehicle's body frame for this message, so the patch simply discards messages with unexpected frames.

\subsection{SA4U's Workflow}
Figure \ref{fig:SA4U_Overview} shows the workflow of SA4U. In step 1, SA4U's instrumentation tool adds logging statements to the firmware's source code. Then, developers build and run the firmware in a simulation. During the simulation, the instrumentation added in step 1 writes a trace file. The developer provides the trace file to SA4U's type deduction tool in step 3. The type deduction tool generates a type database that contains likely types of program variables in the trace file. The type database is augmented with type information from a protocol file that describes the types of fields in the messages exchanged between the pilot's control computer and the UAS. Then, SA4U's static analysis tool uses the type database to check the firmware's original source code. The remainder of this section illustrates the function of these components on our motivating example.

% \subsubsection{Instrumentation} The developer starts by running SA4U's instrumentation program. Instrumentation records the runtime values of program variables for input to the type deduction phase. Figure \ref{fig:Instrumented_Source_Code} shows an example of the instrumented source code. SA4U instruments the assignment to \code{est\_rmt\_time} since it is not a local variable. The instrumentation replaces the original assignment with an invocation of the \code{\_instrument} macro. The parameters passed to \code{\_instrument} are the type of the expression, a number to identify the variable being assigned to, the original expression, and a nonce for hygienic expansion. \code{\_instrument} expands to a statement expression whose body records the value of the assignment expression. The statement expression evaluates to the lvalue of the original destination of the assignment. This allows recursive instrumentation of chained assignment expressions (e.g. \code{x = y = z}.)

\subsubsection{Instrumentation} The developer starts by running SA4U's instrumentation program. Instrumentation records the runtime values of program variables for input to the type deduction phase. Figure \ref{fig:Instrumented_Source_Code} shows an example of the instrumented source code. SA4U instruments the assignments to \lstinline{_angle} and \lstinline{_distance} on lines \ref{fig:Instrumented_Source_Code:instr_1} and \ref{fig:Instrumented_Source_Code:instr_2} since they are not local variables. SA4U skips instrumenting local variables since their types can often be inferred based on their interaction with global variables, and instrumentation disturbs the execution of the firmware. The instrumentation replaces the original assignment with an invocation of the \lstinline{_instrument} macro. The parameters passed to \lstinline{_instrument} are the \emph{linguistic} type of the expression (e.g., \lstinline{int}) encoded as an integer, a number to identify the variable being assigned to, the original expression, and a nonce for hygienic expansion. \lstinline{_instrument} expands to a statement expression whose body records the value of the assignment expression. The statement expression evaluates to the lvalue of the original destination of the assignment. This allows recursive instrumentation of chained assignment expressions (e.g. \lstinline{x = y = z}.)

\subsubsection{Simulation} Next, the developer compiles and runs the instrumented source code with a workload to obtain a trace file. We use the test flights that developers use for debugging as our workloads. The instrumentation that was inserted in the firmware the previous step creates a CSV file that contains the runtime values of program variables. We also manually insert code into the simulator itself to track certain \emph{quantities of interest} whose values are compared with program variables. Examples include latitude, longitude, altitude, velocity, angle adn distance between obstacles, and system time. These values are also written to the trace file.

\subsubsection{Type Deduction}
% The developer provides the trace file produced by the simulation step to SA4U's type deduction program. The type deduction program outputs likely types based on the runtime values of program variables. The type deduction program accomplishes this by comparing program variables to the quantities of interest in the trace file. For example, the value of \code{est\_rmt\_time} is deduced to be a UNIX timestamp because its value is closest to the system's current UNIX time. Note that Section \ref{subsec:Type_Deduction} describes this process more technically. 

The developer provides the trace file produced by the simulation step to SA4U's type deduction program. The type deduction program outputs likely types based on the runtime values of program variables. The type deduction program accomplishes this by comparing program variables to the quantities of interest in the trace file. For example, the type deduction program deduces the value of \lstinline{_angle} is measured in degrees relative to the front of the UAS since \lstinline{_angle} is always nearly equal to a quantity of interest that tracks the heading between the UAS and an obstacle. This data is written to the \emph{type database} that contains the types of program variables. \S \ref{subsec:Type_Deduction} elaborates on how this is accomplished. In contrast, prior work relied on burdensome developer annotations to build a type database.

\subsubsection{Static Analysis}
% Finally, the developer runs the static analysis program. The inputs to the static analysis program are the types that were deduced in the previous step, and a protocol definition file that describes the interface between the pilot's control computer and the UAS. Consider the behavior of the static analysis stage on our motivating example. The program examines the message handler shown on line \ref{fig:Instrumented_Source_Code:1} in Figure \ref{fig:Instrumented_Source_Code}. SA4U knows that the type of \code{e.usec} is a timestamp in either UNIX format or time since system boot because it is defined in the message definition file. SA4U propagates this information across the call graph to \code{correct\_time}. In \code{correct\_time}, the expression \code{est\_rmt\_time - rmt} is marked as a bug, since \code{rmt} is possibly not in the same format as \code{est\_rmt\_time}.

Finally, the developer runs the static analysis program. The inputs to the static analysis program are the type database from the previous stage, a protocol definition file that describes the interface between the pilot's control computer and the UAS, and the firmware source code. The type database is augmented based on the protocol definition file. Then, the static analysis stage parses the source code and generates constraints with the type inference rules described in \S \ref{subsec:Static_Analysis}. After all the source code  has been parsed, the Z3 \cite{z3} theorem prover checks that the constraints are satisfiable. The first constraints that are generated assert the types of program variables match the contents of the type database. For example, \lstinline[keepspaces=true]{type(_angle) = (degrees, MAV_FRAME_BODY_FRD)}.

Consider the behavior of the static analysis stage on our motivating example. The program examines the message handler shown on line \ref{fig:Instrumented_Source_Code:1} in Figure \ref{fig:Instrumented_Source_Code}. SA4U knows that the type of \lstinline{msg.angle} is a measurement in degrees in any coordinate frame because it is defined in the message definition file. After parsing line \ref{fig:Instrumented_Source_Code:2}, SA4U generates the constraint \lstinline[keepspaces=true]{ArgType(set_obstacle_boundary, 1) = (degrees, Any)}. Eventually, SA4U encounters the assignment on line \ref{fig:Instrumented_Source_Code:angle_assgn}. For the assignment to be legal, the type of \lstinline{_angle} must be the same as the \lstinline{angle} parameter. So, SA4U generates the constraint that \lstinline[keepspaces=true]{ArgType(set_obstacle_boundary, 1) = type(_angle)}. SA4U invokes Z3 to check if the constraints that it generates are satisfiable. In this case, they are not satisfiable because there is a contradiction after simplifying: \lstinline[keepspaces=true]{ArgType(set_obstacle_boundary, 1) = (degrees, MAV_FRAME_BODY_FRD)} and \lstinline[keepspaces=true]{ArgType(set_obstacle_boundary, 1) = (degrees, Any)}. Since Z3 reports that the constraints are unsatisfiable, SA4U reports that it has found a bug.

SA4U performs limited interpretation of the source code to avoid false positives. Consider the \textbf{patched} code in Figure \ref{fig:Instrumented_Source_Code}. Existing approaches do not track values of \lstinline{msg.frame}, and so they report a false positive. SA4U solves this problem by partially interpreting the source code. When SA4U sees the conditional statement on line \ref{fig:Instrumented_Source_Code:patch}, SA4U generates the constraint \lstinline[keepspaces=true]{frame(msg.angle) = MAV_FRAME_BODY_FRD}. Then, Z3 \textbf{can} satisfy the constraints, and so SA4U does not incorrectly report a bug.

==> vi_discussion.tex <==
\section{Discussion}

\subsection{Soundness}
SA4U is not sound for several reasons. First, the type deduction phase can derive an incorrect type for a program variable. For example, the program variable \code{emergency\_mode\_alt} could be assigned the type centimeter, when the actual type is meter. When this occurs, SA4U's static analysis phase reports a false positive. Second, the static analysis phase itself is not sound. For example, developers use conversion functions to transform the types of values. SA4U is not aware of all conversion functions, so it misdiagnoses values whose types that are transformed this way. 

\subsection{Completeness}
SA4U is not complete. Once again, the type deduction phase could incorrectly label the type of a program variable. If this occurs, the static analysis phase could fail to diagnose a UTE. Moreover, the static analysis phase can only detect errors if a sufficiently large number of types have been inferred. 
